Cache-based Multi-query Optimization for Data-intensive Scalable Computing Frameworks

In modern large-scale distributed systems, analytics jobs submitted by various users often share similar work, for example scanning and processing the same subset of data. Instead of optimizing jobs independently, which may result in redundant and wasteful processing, multi-query optimization techniques can be employed to save a considerable amount of cluster resources. In this work, we introduce a novel method combining in-memory cache primitives and multi-query optimization, to improve the efficiency of data-intensive, scalable computing frameworks. By careful selection and exploitation of common (sub)expressions, while satisfying memory constraints, our method transforms a batch of queries into a new, more efficient one which avoids unnecessary recomputations. To find feasible and efficient execution plans, our method uses a cost-based optimization formulation akin to the multiple-choice knapsack problem. Extensive experiments on a prototype implementation of our system show significant benefits of worksharing for both TPC-DS workloads and detailed micro-benchmarks.

==> 08_appendices.tex <==
\subsection{TPC-DS sharing}
\label{sec:tpcds-sharing}

We discuss the optimization opportunities and challenges through the following example of 3 queries (Query 3, 43 and 55) from the TPC-DS benchmark \cite{tpcds}:
\begingroup
\fontsize{6pt}{7pt}
\selectfont
\begin{verbatim}
Query 3:
SELECT d_year, i_brand_id, i_brand, sum(ss_ext_sales_price) AS sum_agg
FROM  date_dim, store_sales, item
WHERE d_date_sk = ss_sold_date_sk
AND ss_item_sk = i_item_sk
AND i_manufact_id = 128
AND d_moy=11
GROUP BY d_year, i_brand, i_brand_id
ORDER BY d_year, sum_agg desc, i_brand_id
LIMIT 100

Query 55:
SELECT i_brand_id, i_brand, 
sum(ss_ext_sales_price) ext_price
FROM date_dim, store_sales, item
WHERE d_date_sk = ss_sold_date_sk
AND ss_item_sk = i_item_sk
AND i_manager_id=28
AND d_moy=11
AND d_year=1999
GROUP BY i_brand, i_brand_id
ORDER BY ext_price desc, i_brand_id
LIMIT 100

Query 43:
SELECT s_store_name, s_store_id, 
sum(case when (d_day_name='Sunday') 
then ss_sales_price else null end) sun_sales,
sum(case when (d_day_name='Monday') 
then ss_sales_price else null end) mon_sales,
...
sum(case when (d_day_name='Saturday') 
then ss_sales_price else null end) sat_sales
FROM date_dim, store_sales, store
WHERE d_date_sk = ss_sold_date_sk 
AND s_store_sk = ss_store_sk
AND s_gmt_offset = -5
AND d_year = 2000
GROUP BY s_store_name, s_store_id
ORDER BY s_store_name, s_store_id,sun_sales,mon_sales,tue_sales,
wed_sales, thu_sales,fri_sales,sat_sales
LIMIT 100
\end{verbatim}
\endgroup

\begin{figure*}[htbp]
	\centering
	\includegraphics[scale=0.5]{figures/q3}
	\includegraphics[scale=0.5]{figures/q55}
	\includegraphics[scale=0.5]{figures/q43}
	\caption{Optimized operator trees of query 3, 55 and 43 (from left to right) in the TPC-DS benchmark} 
	\label{fig:queries}
\end{figure*}
